TREE-G: Decision Trees Contesting Graph Neural Networks

When dealing with tabular data, models based on decision trees are a popular choice due to their high accuracy on these data types, their ease of application, and explainability properties. However, when it comes to graph-structured data, it is not clear how to apply them effectively, in a way that incorporates the topological information with the tabular data available on the vertices of the graph. To address this challenge, we introduce TREE-G. TREE-G modifies standard decision trees, by introducing a novel split function that is specialized for graph data. Not only does this split function incorporate the node features and the topological information, but it also uses a novel pointer mechanism that allows split nodes to use information computed in previous splits. Therefore, the split function adapts to the predictive task and the graph at hand. We analyze the theoretical properties of TREE-G and demonstrate its benefits empirically on multiple graph and vertex prediction benchmarks. In these experiments, TREE-G consistently outperforms other tree-based models and often outperforms other graph-learning algorithms such as Graph Neural Networks (GNNs) and Graph Kernels, sometimes by large margins. Moreover, TREE-Gs models and their predictions can be explained and visualized

==> feature_engineering_lemma_proof.tex <==
\begin{lemma*}
An implementation of \acronym in a non-dynamic approach where all the dynamic features are computed in advance, requires a computation that is exponential in the number of input features.
\end{lemma*}

To prove that, recall that in \acronym each split-node $v$ generates exactly two subsets, which are defined over the selected input feature $k$, $1\leq k \leq m$, and the available subsets. The available subsets are at most $2D$ subsets, generated in the $D-1$ previous splits in path path from $v$ to the root.
In particular, when generating the subset in node $v$ of depth $D$, the selected feature $k$ is already known.
Nevertheless this is not the case if the dynamic features are computed in advance instead of the incremental approach in \acronym.
The key insight is that in advance it is not known what the selected input features $k$ and subset $S_{u, \rho}$ will be in every split node. 
Therefore,  just to mimic the generation of subsets in a split node of depth $D$, we have to compute all the subsets that could, potentially, be generated in \acronym. We call these subset \textir{potentially generated subsets} and show that in a node of depth $D$, their amount is $m^{D-1}$ .
% in advance, one will have to consider all possible subsets defined over all possible combination of input features. 
% We show that that number of possible subsets that may be considered in a split-node of depth $D$ is $\Theta(m^{D-1})$. 
% Therefore, just to compute all possible the subsets that may be used in split-node of depth $D$, an exponential number of computation in $m$ is required.
% Each of the two subsets generated in the previous $D-1$ split node, is dependent on the selected input feature $1\leq k \leq m$ in that split. In \acronym the subsets are computed incrementally. Therefore, in depth $D$, the $2D$ generated subsets are already known. 
% If all subsets are computed in advances, there are exponential many.
% This is because a subset considered in depth $D$, is dependent on $D-1$ input features that were chosen above in the tree.Clearly in advance, it is not known  which $D-1$ input feature will be chosen.
% Therefore, we show that that number of possible subsets that may be considered in a split-node of depth $D$ is $\Theta(m^{D-1})$. 
% Therefore, just to compute all possible the subsets that may be used in split-node of depth $D$, an exponential number of computation in $m$ is required.


% It is important to note that in \acronym we use a dynamic approach, and the subset are computed incrementally. Therefore, in depth $D$, the $D$ input features that were already selected in previous splits are know and the selected subset are already known, and therefore only linear amount of subsets needs to be considered. 
We prove the following claim:
\begin{lemma*}
The number of potentially generated subsets in a split node of depth $v$ is $\Omega\left(m^{D-1}\right)$. 
\end{lemma*}

We prove this by induction on $D$.
If $D=1$ then the tree is composed from just a root. The used subset in the root is contains only the set of vertices $V$.  There are $m$ input features, each corresponds to two generates subsets. Therefore, the number of potentially generated subsets is $2m = \Omega\left(m^1\right)$. 
Now assume that the number of potentially generated in a split-node of depth $D-1$ is $\Omega\left(m^{D-1}\right)$.
Let $v$ be a split-node of depth $D$.
The selected subset in $v$ may be one from the generated subsets in its parent node. Its parent node is of depth $D-1$ and therefore it has $\Omega\left(m^{D-1}\right)$ potentially generated subsets.
There are $m$ input features, each corresponds to two generates subsets in $v$.  Therefore, the number of potentially generated subsets in $v$ is $m\cdot \Omega\left(m^{D-1}\right) = \Omega\left(m^D\right)$.


